Factorization and Color-Suppression in Hadronic B->D^(*)npi Decays

The factorization hypothesis and color-suppression are investigated by analyzing the largest, to date, sample of B mesons. In all, 20 hadronic two-body decay modes are reconstructed using 2.04 fb^-1 of data collected with the CLEOII detector. We measure the branching fraction of five class I and five class III decay modes and set upper limits on branching fractions of ten class II decays. The branching fraction measurements are used to determine the BSW parameters a_1, and a_2/a_1. In addition, we measure the fraction of B-> D^{*+} rho^- decays which decay longitudinally polarized. The results are found to be consistent with factorization and color-suppression.

==> tbl_colorsup.tex <==
%auto-ignore    
\TableTitle\tblcoloratio{Table of ratio of class II to class I $B$ decays} 

{\begintable

Ratio of {\cal B} & U.L. & BSWII & CDDFGN || Ratio of {\cal B} & U.L.  & BSWII & CDDFGN  \cr
${{\cal B}(B^0\to D^0\pi^0)\over{\cal B}(B^0\to D^+\pi^-)}$      \hfill&$<0.11$&$0.0129$&$0.0406$||${{\cal B}(B^0\to D^{*0}\pi^0)\over{\cal B}(B^0\to D^{*+}\pi^-)}$      \hfill& $< 0.18 $& $0.0134$      &$0.0328$\crnorule
${{\cal B}(B^0\to D^0\eta)\over{\cal B}(B^0\to D^+\pi^-)}$       \hfill&$<0.11$&$     $	&$0.0119$||${{\cal B}(B^0\to D^{*0}\eta)\over{\cal B}(B^0\to D^{*+}\pi^-)}$       \hfill& $< 0.16 $& $0.0176$      &$0.0079$\crnorule
${{\cal B}(B^0\to D^0\eta^\prime)\over{\cal B}(B^0\to D^+\pi^-)}$\hfill&$<0.09$&$0.0019$     &$$ ||${{\cal B}(B^0\to D^{*0}\eta^\prime)\over{\cal B}(B^0\to D^{*+}\pi^-)}$\hfill& $< 0.44 $& $0.0020$      &$$\crnorule      
${{\cal B}(B^0\to D^0\rho^0)\over{\cal B}(B^0\to D^+\rho^-)}$    \hfill&$<0.07$&$0.0037$&$0.0024$||${{\cal B}(B^0\to D^{*0}\rho^0)\over{\cal B}(B^0\to D^{*+}\rho^-)}$    \hfill& $< 0.14 $& $0.0033$      &$0.0064$\crnorule
${{\cal B}(B^0\to D^0\omega)\over{\cal B}(B^0\to D^+\rho^-)}$    \hfill&$<0.07$&$0.0072$&$0.0024$||${{\cal B}(B^0\to D^{*0}\omega)\over{\cal B}(B^0\to D^{*+}\rho^-)}$    \hfill& $< 0.14 $& $0.0064$      &$0.0064$         





\endtable}
\bigtype
\TableCaption{Note: The values of $a_2/a_1$ used are from Equation \(a2overa1).}



